The As-If Machine: Personalized AI counterfactuals make distant policy risks feel close

Life experiences can shape policy attitudes, but we only live one life. Citizens may therefore fail to support policies addressing risks they have never personally experienced. Narratives can make such risks immediate and personal, but personalized stories remain difficult to produce at scale. Here we ask whether AI can make distant scenarios feel concrete by simulating a participant's life as if that scenario occurred. We present the As-If Machine (AIM), a multi-agent system through which people co-write personalized counterfactual narratives---stories about their own lives under different policy futures. In two pre-registered and quota-matched experiments on science funding (N=1,007) and satellite cybersecurity (N=894), we compared AIM with two controls: reading an expert-written vignette on the same topic and co-writing with AIM about an unrelated topic. AIM increased psychological closeness---how close a risk feels to the self---by nearly identical margins in the two domains (0.36 and 0.38 standard deviations (SDs) against the vignette, 0.80 and 0.90 against unrelated writing). AIM increased psychological closeness even among participants with unfavorable views of AI. For policy attitudes, AIM's effects were 0.16 SDs against the vignette and 0.10 SDs (n.s.) against unrelated writing for science funding; the corresponding effects for satellite cybersecurity were 0.54 and 0.67 SDs. Across 23,496 human-AI autocomplete interactions, participants and the system played distinct roles: AIM supplied concrete detail that grounded the scenario, and participants supplied first-person perspective and emotion. Co-writing with the As-If Machine makes distant policy risks feel close.

==> explain_divergence/tables/crystallization.tex <==
\begin{table}[H]
\caption{Ideology predicting attitudes in the control arms, before any exposure to AIM.}
\label{tab:crystallization}
\begin{tabular}{llrrrrr}
\toprule
study & predictor & b & lo & hi & p & n \\
\midrule
Study 1 & Ideological direction & -0.181 & -0.273 & -0.088 & 0.000 & 674 \\
Study 1 & Ideological strength & 0.097 & 0.022 & 0.172 & 0.011 & 674 \\
Study 2 & Ideological direction & 0.086 & -0.004 & 0.177 & 0.061 & 596 \\
Study 2 & Ideological strength & -0.024 & -0.111 & 0.063 & 0.583 & 596 \\
\bottomrule
\end{tabular}
\end{table}


==> explain_divergence/tables/ruled_out_items.tex <==
\begin{table}[H]
\caption{AIM effects on each Study 1 attitude item. Each item is z-scored within Study 1; each effect is AIM minus the control in standard deviations, from a model of the item on arm with HC1 standard errors. The attitude index averages the two standardized items.}
\label{tab:ruled_out_items}
\begin{tabular}{lllllr}
\toprule
Outcome & AIM vs vignette [95\% CI] & p (vignette) & AIM vs placebo [95\% CI] & p (placebo) & n \\
\midrule
Attitude index & 0.16 [0.00, 0.32] & .045 & 0.10 [-0.05, 0.24] & .191 & 1007 \\
Personal benefit of U.S. science (1-5) & 0.12 [-0.03, 0.27] & .122 & 0.02 [-0.13, 0.16] & .832 & 1007 \\
Preferred NIH share of federal spending (0-100) & 0.10 [-0.05, 0.26] & .191 & 0.12 [-0.03, 0.27] & .107 & 1007 \\
\bottomrule
\end{tabular}
\end{table}


==> explain_divergence/tables/share_explained.tex <==
\begin{table}[H]
\caption{Percent of the Study 2 minus Study 1 difference in the AIM effect on attitudes that closes when Study 1 is given the Study 2 value of each path parameter. Intervals resample participants within study and arm.}
\label{tab:share_explained}
\begin{tabular}{llrrr}
\toprule
control & substitution & pct_gap_closed & lo & hi \\
\midrule
vignette & Closeness conversion & 4.354 & -10.177 & 23.670 \\
vignette & Transportation engagement & 9.497 & 1.414 & 23.890 \\
vignette & Transportation conversion & 4.153 & -1.994 & 18.512 \\
vignette & Transportation, both paths & 24.359 & 10.121 & 54.545 \\
vignette & All three identified paths & 28.713 & 12.052 & 63.901 \\
vignette & Remainder (direct path) & 71.287 & NaN & NaN \\
placebo & Closeness conversion & 24.018 & 8.544 & 48.348 \\
placebo & Transportation engagement & 5.421 & 0.317 & 11.969 \\
placebo & Transportation conversion & 0.032 & -2.295 & 2.153 \\
placebo & Transportation, both paths & 7.665 & 1.010 & 15.948 \\
placebo & All three identified paths & 31.682 & 15.063 & 56.608 \\
placebo & Remainder (direct path) & 68.318 & NaN & NaN \\
\bottomrule
\end{tabular}
\end{table}


==> explain_divergence/tables/transportation_items.tex <==
\begin{table}[H]
\caption{Treatment effect on each transportation item, on the administered 1-7 scale.}
\label{tab:transportation_items}
\begin{tabular}{lllrrrrr}
\toprule
study & control & item & b & lo & hi & p & n \\
\midrule
Study 1 & vignette & Pictured self & 0.762 & 0.542 & 0.982 & 0.000 & 664 \\
Study 1 & vignette & Mentally involved & 0.416 & 0.236 & 0.596 & 0.000 & 664 \\
Study 1 & vignette & Wanted to learn more & -0.149 & -0.353 & 0.056 & 0.155 & 664 \\
Study 1 & vignette & Emotionally affected & -0.547 & -0.820 & -0.274 & 0.000 & 664 \\
Study 1 & placebo & Pictured self & 0.123 & -0.077 & 0.324 & 0.228 & 676 \\
Study 1 & placebo & Mentally involved & -0.013 & -0.179 & 0.154 & 0.883 & 676 \\
Study 1 & placebo & Wanted to learn more & -0.222 & -0.427 & -0.017 & 0.034 & 676 \\
Study 1 & placebo & Emotionally affected & 0.126 & -0.147 & 0.398 & 0.365 & 676 \\
Study 2 & vignette & Pictured self & 0.912 & 0.677 & 1.147 & 0.000 & 601 \\
Study 2 & vignette & Mentally involved & 0.386 & 0.200 & 0.572 & 0.000 & 601 \\
Study 2 & vignette & Wanted to learn more & -0.048 & -0.268 & 0.172 & 0.668 & 601 \\
Study 2 & vignette & Emotionally affected & 0.477 & 0.189 & 0.766 & 0.001 & 601 \\
Study 2 & placebo & Pictured self & 0.483 & 0.267 & 0.699 & 0.000 & 591 \\
Study 2 & placebo & Mentally involved & 0.140 & -0.032 & 0.312 & 0.110 & 591 \\
Study 2 & placebo & Wanted to learn more & 0.022 & -0.198 & 0.243 & 0.842 & 591 \\
Study 2 & placebo & Emotionally affected & 0.411 & 0.119 & 0.703 & 0.006 & 591 \\
\bottomrule
\end{tabular}
\end{table}


==> satellite/tables/satellite_sensitivity.tex <==
\begin{table}
\caption{Satellite sensitivity analysis excluding five records without linked Prolific data.}
\label{tab:sensitivity}
\begin{tabular}{lllrrrr}
\toprule
Sample & Outcome & Control & $n$ & $b$ & 95\% CI & $p$ \\
\midrule
Retained sample & Closeness & Vignette & 894 & 0.379 & [0.243, 0.515] & $4.55\times10^{-8}$ \\
Retained sample & Closeness & Placebo & 894 & 0.896 & [0.744, 1.048] & $7.8\times10^{-31}$ \\
Retained sample & Attitude & Vignette & 894 & 0.544 & [0.393, 0.695] & $1.72\times10^{-12}$ \\
Retained sample & Attitude & Placebo & 894 & 0.666 & [0.517, 0.816] & $2.18\times10^{-18}$ \\
Prolific-matched & Closeness & Vignette & 889 & 0.374 & [0.238, 0.511] & $7.57\times10^{-8}$ \\
Prolific-matched & Closeness & Placebo & 889 & 0.891 & [0.738, 1.044] & $3.59\times10^{-30}$ \\
Prolific-matched & Attitude & Vignette & 889 & 0.535 & [0.384, 0.687] & $4.27\times10^{-12}$ \\
Prolific-matched & Attitude & Placebo & 889 & 0.663 & [0.513, 0.813] & $5.04\times10^{-18}$ \\
\bottomrule
\end{tabular}
\end{table}


==> satellite/tables/tab_balance.tex <==
\begin{table}
\caption{Study 2 (satellite cybersecurity) participant descriptives by arm: pre-treatment covariates (M (SD) for continuous; \% for binary). One-way ANOVA $F$-tests for continuous variables; $\chi^2$ for binary. Party ID (Democrat / Independent / Republican) is a $\chi^2$ test on participants with Prolific party data, missing for 6 participants. $q$ is the sharpened false-discovery-rate $q$ value, correcting for multiple comparisons across covariates.}
\label{tab:balance_satellite}
\begin{tabular}{llllll}
\toprule
Variable & Treat & Placebo & Vignette & Test & q \\
\midrule
Age & 45.81 (15.23) & 45.61 (14.65) & 47.29 (14.36) & F=1.17 & 0.329 \\
Male (\%) & 40.9\% & 46.8\% & 49.2\% & $\chi^2$=4.33 & 0.221 \\
Education (Recoded 1–8) & 3.27 (1.13) & 3.22 (1.10) & 3.18 (1.04) & F=0.48 & 0.567 \\
Income (Recoded 1–7) & 4.29 (1.89) & 4.10 (1.81) & 3.87 (1.86) & F=3.78 & 0.133 \\
Political Ideology (+ = conservative) & 3.56 (1.72) & 3.83 (1.76) & 3.82 (1.85) & F=2.21 & 0.221 \\
Familiarity w/ satellite cybersecurity & 2.72 (1.60) & 2.80 (1.51) & 3.05 (1.55) & F=3.72 & 0.133 \\
Mental imagery & 8.58 (1.42) & 8.57 (1.49) & 8.65 (1.39) & F=0.26 & 0.712 \\
IRI Fantasy & 3.80 (0.87) & 3.69 (0.86) & 3.73 (0.94) & F=1.15 & 0.329 \\
IRI Perspective-taking & 3.86 (0.87) & 3.92 (0.83) & 3.95 (0.86) & F=0.87 & 0.416 \\
IRI Personal distress & 2.61 (0.96) & 2.44 (0.93) & 2.53 (0.95) & F=2.40 & 0.221 \\
Creative writing exp. & 3.37 (1.06) & 3.12 (1.05) & 3.29 (1.07) & F=4.02 & 0.133 \\
Journaling freq. & 3.08 (1.13) & 2.89 (1.15) & 2.91 (1.16) & F=2.51 & 0.221 \\
AI attitudes & 6.69 (2.30) & 6.76 (2.25) & 6.73 (2.29) & F=0.08 & 0.856 \\
Party ID: D / I / R (\%) & 31.4 / 44.3 / 24.3 & 26.1 / 44.0 / 29.9 & 27.2 / 43.5 / 29.2 & $\chi^2$=3.62 & 0.416 \\
\bottomrule
\end{tabular}
\end{table}


==> sci_fund_real/tables/tab_balance.tex <==
\begin{table}
\caption{Study 1 (science funding) participant descriptives by arm: pre-treatment covariates (M (SD) for continuous; \% for binary). One-way ANOVA $F$-tests for continuous variables; $\chi^2$ for binary. Party ID (Democrat / Independent / Republican) is a $\chi^2$ test on participants with Prolific party data, missing for 5 participants. $q$ is the sharpened false-discovery-rate $q$ value, correcting for multiple comparisons across covariates.}
\label{tab:balance_science}
\begin{tabular}{llllll}
\toprule
Variable & Treat & Placebo & Vignette & Test & q \\
\midrule
Age & 45.62 (15.43) & 45.39 (15.36) & 45.70 (15.69) & F=0.04 & 1.000 \\
Male (\%) & 45.9\% & 47.2\% & 49.8\% & $\chi^2$=1.05 & 1.000 \\
Education (Recoded 1–8) & 3.15 (0.98) & 3.16 (1.14) & 3.25 (1.29) & F=0.81 & 1.000 \\
Income (Recoded 1–7) & 4.06 (1.90) & 4.22 (1.93) & 4.38 (1.82) & F=2.38 & 1.000 \\
Political Ideology (+ = conservative) & 3.63 (1.79) & 3.71 (1.75) & 3.83 (1.83) & F=1.06 & 1.000 \\
Familiarity w/ sci. funding & 2.87 (1.54) & 2.76 (1.49) & 2.82 (1.54) & F=0.42 & 1.000 \\
Mental imagery & 8.69 (1.25) & 8.56 (1.42) & 8.60 (1.40) & F=0.77 & 1.000 \\
IRI Fantasy & 3.69 (0.95) & 3.71 (0.93) & 3.69 (0.90) & F=0.10 & 1.000 \\
IRI Perspective-taking & 3.90 (0.83) & 3.86 (0.87) & 3.90 (0.82) & F=0.30 & 1.000 \\
IRI Personal distress & 2.59 (0.92) & 2.57 (0.97) & 2.50 (0.94) & F=0.89 & 1.000 \\
Creative writing exp. & 3.08 (1.10) & 3.12 (1.08) & 2.99 (1.16) & F=1.07 & 1.000 \\
Journaling freq. & 2.88 (1.14) & 2.81 (1.13) & 2.80 (1.18) & F=0.42 & 1.000 \\
AI attitudes & 6.51 (2.38) & 6.80 (2.15) & 6.62 (2.29) & F=1.47 & 1.000 \\
Party ID: D / I / R (\%) & 27.5 / 46.2 / 26.3 & 27.9 / 44.4 / 27.6 & 27.8 / 43.8 / 28.4 & $\chi^2$=0.52 & 1.000 \\
\bottomrule
\end{tabular}
\end{table}


==> study_comparison/tables/tab_mediator_partial_correlations.tex <==
\begin{longtable}{llrll}
\caption{Correlation between closeness and transportation before and after partialling out treatment.} \label{tab:mediator_partial_correlations} \\
\toprule
Study & Control & $n$ & $r$ & Partial $r$ [95\% CI] \\
\midrule
\endfirsthead
\caption[]{Correlation between closeness and transportation before and after partialling out treatment.} \\
\toprule
Study & Control & $n$ & $r$ & Partial $r$ [95\% CI] \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Pooled & Vignette & 1265 & +0.524 & +0.515 [+0.47, +0.55] \\
Study 1 & Vignette & 664 & +0.491 & +0.492 [+0.43, +0.55] \\
Study 2 & Vignette & 601 & +0.562 & +0.544 [+0.48, +0.60] \\
\end{longtable}


==> study_comparison/tables/tab_parallel_effects.tex <==
\begin{longtable}{llll}
\caption{Parallel multiple-mediator effects, with residual covariance free rather than fixed at zero, with 95\% bias-corrected bootstrap intervals.} \label{tab:parallel_effects} \\
\toprule
Study & Control & Effect & Estimate [95\% CI] \\
\midrule
\endfirsthead
\caption[]{Parallel multiple-mediator effects, with residual covariance free rather than fixed at zero, with 95\% bias-corrected bootstrap intervals.} \\
\toprule
Study & Control & Effect & Estimate [95\% CI] \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Pooled & Vignette & Via closeness & +0.153 [+0.106, +0.210] \\
Pooled & Vignette & Via transportation & +0.050 [+0.024, +0.082] \\
Pooled & Vignette & Total indirect & +0.202 [+0.141, +0.267] \\
Pooled & Vignette & Total & +0.342 [+0.227, +0.457] \\
Pooled & Vignette & Direct & +0.140 [+0.039, +0.240] \\
Pooled & Placebo & Via closeness & +0.380 [+0.316, +0.449] \\
Pooled & Placebo & Via transportation & +0.019 [+0.001, +0.041] \\
Pooled & Placebo & Total indirect & +0.399 [+0.328, +0.477] \\
Pooled & Placebo & Total & +0.363 [+0.253, +0.465] \\
Pooled & Placebo & Direct & -0.036 [-0.151, +0.058] \\
Pooled & Pooled & Via closeness & +0.256 [+0.203, +0.297] \\
Pooled & Pooled & Via transportation & +0.037 [+0.016, +0.061] \\
Pooled & Pooled & Total indirect & +0.292 [+0.233, +0.346] \\
Pooled & Pooled & Total & +0.353 [+0.260, +0.445] \\
Pooled & Pooled & Direct & +0.060 [-0.018, +0.147] \\
Study 1 & Vignette & Via closeness & +0.141 [+0.076, +0.212] \\
Study 1 & Vignette & Via transportation & +0.014 [-0.004, +0.048] \\
Study 1 & Vignette & Total indirect & +0.155 [+0.081, +0.231] \\
Study 1 & Vignette & Total & +0.160 [-0.003, +0.315] \\
Study 1 & Vignette & Direct & +0.005 [-0.145, +0.149] \\
Study 1 & Placebo & Via closeness & +0.297 [+0.219, +0.382] \\
Study 1 & Placebo & Via transportation & +0.000 [-0.020, +0.024] \\
Study 1 & Placebo & Total indirect & +0.297 [+0.208, +0.386] \\
Study 1 & Placebo & Total & +0.098 [-0.059, +0.241] \\
Study 1 & Placebo & Direct & -0.199 [-0.358, -0.061] \\
Study 1 & Pooled & Via closeness & +0.216 [+0.162, +0.275] \\
Study 1 & Pooled & Via transportation & +0.008 [-0.011, +0.031] \\
Study 1 & Pooled & Total indirect & +0.224 [+0.158, +0.293] \\
Study 1 & Pooled & Total & +0.128 [-0.008, +0.260] \\
Study 1 & Pooled & Direct & -0.096 [-0.225, +0.030] \\
Study 2 & Vignette & Via closeness & +0.168 [+0.103, +0.242] \\
Study 2 & Vignette & Via transportation & +0.108 [+0.058, +0.179] \\
Study 2 & Vignette & Total indirect & +0.275 [+0.179, +0.384] \\
Study 2 & Vignette & Total & +0.544 [+0.397, +0.697] \\
Study 2 & Vignette & Direct & +0.268 [+0.151, +0.404] \\
Study 2 & Placebo & Via closeness & +0.485 [+0.373, +0.590] \\
Study 2 & Placebo & Via transportation & +0.044 [+0.014, +0.084] \\
Study 2 & Placebo & Total indirect & +0.529 [+0.412, +0.637] \\
Study 2 & Placebo & Total & +0.666 [+0.503, +0.810] \\
Study 2 & Placebo & Direct & +0.138 [-0.000, +0.272] \\
Study 2 & Pooled & Via closeness & +0.305 [+0.233, +0.379] \\
Study 2 & Pooled & Via transportation & +0.079 [+0.043, +0.125] \\
Study 2 & Pooled & Total indirect & +0.384 [+0.296, +0.468] \\
Study 2 & Pooled & Total & +0.604 [+0.492, +0.724] \\
Study 2 & Pooled & Direct & +0.220 [+0.122, +0.323] \\
\end{longtable}


==> study_comparison/tables/tab_serial_effects.tex <==
\begin{longtable}{llll}
\caption{Serial multiple-mediator effects with 95\% bias-corrected bootstrap intervals.} \label{tab:serial_effects} \\
\toprule
Study & Control & Effect & Estimate [95\% CI] \\
\midrule
\endfirsthead
\caption[]{Serial multiple-mediator effects with 95\% bias-corrected bootstrap intervals.} \\
\toprule
Study & Control & Effect & Estimate [95\% CI] \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Pooled & Vignette & Via closeness & +0.153 [+0.106, +0.210] \\
Pooled & Vignette & Via transportation & +0.002 [-0.019, +0.026] \\
Pooled & Vignette & Via closeness $\rightarrow$ transportation & +0.047 [+0.030, +0.068] \\
Pooled & Vignette & Total indirect & +0.202 [+0.141, +0.267] \\
Pooled & Vignette & Total & +0.342 [+0.227, +0.457] \\
Pooled & Vignette & Direct & +0.140 [+0.039, +0.240] \\
Pooled & Placebo & Via closeness & +0.380 [+0.316, +0.449] \\
Pooled & Placebo & Via transportation & -0.026 [-0.047, -0.006] \\
Pooled & Placebo & Via closeness $\rightarrow$ transportation & +0.045 [+0.030, +0.064] \\
Pooled & Placebo & Total indirect & +0.399 [+0.328, +0.477] \\
Pooled & Placebo & Total & +0.363 [+0.253, +0.465] \\
Pooled & Placebo & Direct & -0.036 [-0.151, +0.058] \\
Pooled & Pooled & Via closeness & +0.256 [+0.203, +0.297] \\
Pooled & Pooled & Via transportation & -0.014 [-0.032, +0.006] \\
Pooled & Pooled & Via closeness $\rightarrow$ transportation & +0.051 [+0.038, +0.064] \\
Pooled & Pooled & Total indirect & +0.292 [+0.233, +0.346] \\
Pooled & Pooled & Total & +0.353 [+0.260, +0.445] \\
Pooled & Pooled & Direct & +0.060 [-0.018, +0.147] \\
Study 1 & Vignette & Via closeness & +0.141 [+0.076, +0.212] \\
Study 1 & Vignette & Via transportation & -0.014 [-0.040, +0.002] \\
Study 1 & Vignette & Via closeness $\rightarrow$ transportation & +0.028 [+0.012, +0.056] \\
Study 1 & Vignette & Total indirect & +0.155 [+0.080, +0.231] \\
Study 1 & Vignette & Total & +0.160 [-0.003, +0.315] \\
Study 1 & Vignette & Direct & +0.005 [-0.145, +0.150] \\
Study 1 & Placebo & Via closeness & +0.297 [+0.220, +0.382] \\
Study 1 & Placebo & Via transportation & -0.030 [-0.065, -0.010] \\
Study 1 & Placebo & Via closeness $\rightarrow$ transportation & +0.030 [+0.015, +0.052] \\
Study 1 & Placebo & Total indirect & +0.297 [+0.208, +0.386] \\
Study 1 & Placebo & Total & +0.098 [-0.059, +0.241] \\
Study 1 & Placebo & Direct & -0.199 [-0.358, -0.061] \\
Study 1 & Pooled & Via closeness & +0.216 [+0.162, +0.275] \\
Study 1 & Pooled & Via transportation & -0.026 [-0.051, -0.008] \\
Study 1 & Pooled & Via closeness $\rightarrow$ transportation & +0.034 [+0.021, +0.052] \\
Study 1 & Pooled & Total indirect & +0.224 [+0.159, +0.293] \\
Study 1 & Pooled & Total & +0.128 [-0.007, +0.260] \\
Study 1 & Pooled & Direct & -0.096 [-0.224, +0.030] \\
Study 2 & Vignette & Via closeness & +0.168 [+0.103, +0.242] \\
Study 2 & Vignette & Via transportation & +0.038 [-0.003, +0.086] \\
Study 2 & Vignette & Via closeness $\rightarrow$ transportation & +0.070 [+0.040, +0.111] \\
Study 2 & Vignette & Total indirect & +0.275 [+0.179, +0.384] \\
Study 2 & Vignette & Total & +0.544 [+0.397, +0.697] \\
Study 2 & Vignette & Direct & +0.268 [+0.151, +0.404] \\
Study 2 & Placebo & Via closeness & +0.485 [+0.373, +0.590] \\
Study 2 & Placebo & Via transportation & -0.015 [-0.046, +0.015] \\
Study 2 & Placebo & Via closeness $\rightarrow$ transportation & +0.059 [+0.037, +0.091] \\
Study 2 & Placebo & Total indirect & +0.529 [+0.411, +0.637] \\
Study 2 & Placebo & Total & +0.666 [+0.502, +0.809] \\
Study 2 & Placebo & Direct & +0.138 [-0.000, +0.272] \\
Study 2 & Pooled & Via closeness & +0.305 [+0.233, +0.379] \\
Study 2 & Pooled & Via transportation & +0.011 [-0.020, +0.049] \\
Study 2 & Pooled & Via closeness $\rightarrow$ transportation & +0.069 [+0.049, +0.093] \\
Study 2 & Pooled & Total indirect & +0.384 [+0.296, +0.468] \\
Study 2 & Pooled & Total & +0.604 [+0.492, +0.724] \\
Study 2 & Pooled & Direct & +0.220 [+0.122, +0.322] \\
\end{longtable}

